Study of Adaptive LLR-based AP selection for Grant-Free Random Access in Cell-Free Networks

This paper presents an iterative detection and decoding scheme along with an adaptive strategy to improve the selection of access points (APs) in a grant-free uplink cell-free scenario. With the requirement for the APs to have low-computational power in mind, we introduce a low-complexity scheme for local activity and data detection. At the central processing unit (CPU) level, we propose an adaptive technique based on local log-likelihood ratios (LLRs) to select the list of APs that should be considered for each device. Simulation results show that the proposed LLRs-based APs selection scheme outperforms the existing techniques in the literature in terms of bit error rate (BER) while requiring comparable fronthaul load.

==> fig/FERxSNR.tex <==
\begin{tikzpicture}
\begin{axis}[%
width=6.5cm,
height=4.2cm,
scale only axis,
xmin=-9,
xmax=12.5,
xlabel style={font=\color{white!15!black}},
xlabel={average SNR [dB]},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={FER},
axis background/.style={fill=white},
title style={font=\bfseries, align=center},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.4,0.02)}, font=\footnotesize, anchor=south east, legend cell align=left, align=left, draw=white!15!black},
cycle multi list={Set2-7} % color brewer cycle multi list
]

\addplot [color=\Randomcolor, line width=0.8pt, mark=star,mark size = 1.8pt, mark options={solid, \Randomcolor}]
  table[row sep=crcr]{%
    -9  0.999700000000000\\
    -6  0.989899999999999\\
    -3  0.914999999999998\\
    0   0.674300000000000\\
    3	0.476080000000000\\
    6	0.333000000000000\\
    9   0.166000000000000\\
    12  0.0837000000000000\\
};
\addlegendentry{Random}

% ------------------------------------------
\addplot [color=\LLSFcolor, line width=0.8pt, mark=diamond,mark size = 1.8pt, mark options={solid, \LLSFcolor}]
  table[row sep=crcr]{%
    -9  0.999700000000000\\
    -6  0.989899999999999\\
    -3  0.914999999999998\\
    -0  0.654300000000000\\
    3	0.360800000000000\\
    6	0.0993000000000000\\
    9   0.0366000000000000\\
    12  0.00537000000000000\\
};
\addlegendentry{LLSF}

% ------------------------------------------
\addplot [color=\LECGcolor, line width=0.8pt, mark=square,mark size = 1.5pt, mark options={solid, \LECGcolor}]
  table[row sep=crcr]{%
    -9  0.999700000000000\\
    -6  0.989899999999999\\
    -3  0.914999999999998\\
    -0  0.654300000000000\\
    3	0.330800000000000\\
    6	0.057930000000000\\
    9   0.0126000000000000\\
    12  0.00107000000000000\\
};
\addlegendentry{LECG}

% ------------------------------------------
\addplot [color=\LLRmcolor, line width=0.8pt, mark=o,mark size = 1.5pt, mark options={solid, \LLRmcolor}]
  table[row sep=crcr]{%
    -9  0.999700000000000\\
    -6  0.989799999999999\\
    -3  0.914799999999998\\
    -0  0.652500000000000\\
    3	0.255100000000000\\
    6	0.0421000000000000\\
    9   0.0056000000000000\\
    12  0.0005000000000000\\
};
\addlegendentry{LLR-based}

% ------------------------------------------
\addplot [color=\Allcolor, line width=0.5pt, mark=10-pointed star,mark size = 1.5pt, mark options={solid, \Allcolor}]
  table[row sep=crcr]{%
    -9  0.999700000000000\\
    -6  0.989799999999999\\
    -3  0.914699999999998\\
    -0  0.649900000000000\\
    3	0.252800000000000\\
    6	0.0383000000000000\\
    9   0.0038000000000000\\
    12  0.0003000000000000\\
};
\addlegendentry{All APs}

\end{axis}
\end{tikzpicture}%

